Vehicle: Bridging the Embedding Gap in the Verification of Neuro-Symbolic Programs

Neuro-symbolic programs, i.e. programs containing both machine learning components and traditional symbolic code, are becoming increasingly widespread. Finding a general methodology for verifying such programs is challenging due to both the number of different tools involved and the intricate interface between the ``neural'' and ``symbolic'' program components. In this paper we present a general decomposition of the neuro-symbolic verification problem into parts, and examine the problem of the embedding gap that occurs when one tries to combine proofs about the neural and symbolic components. To address this problem we then introduce Vehicle -- standing as an abbreviation for a ``verification condition language'' -- an intermediate programming language interface between machine learning frameworks, automated theorem provers, and dependently-typed formalisations of neuro-symbolic programs. Vehicle allows users to specify the properties of the neural components of neuro-symbolic programs once, and then safely compile the specification to each interface using a tailored typing and compilation procedure. We give a high-level overview of Vehicle's overall design, its interfaces and compilation & type-checking procedures, and then demonstrate its utility by formally verifying the safety of a simple autonomous car controlled by a neural network, operating in a stochastic environment with imperfect information.

==> agda/initialState.tex <==
\begin{code}%
\>[0]\AgdaFunction{initialState}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\<%
\\
\>[0]\AgdaFunction{initialState}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{state}\AgdaSpace{}%
\AgdaFunction{0ℚ}\AgdaSpace{}%
\AgdaFunction{0ℚ}\AgdaSpace{}%
\AgdaFunction{0ℚ}\AgdaSpace{}%
\AgdaFunction{0ℚ}\<%
\end{code}

==> agda/onRoad.tex <==
\begin{code}%
\>[0]\AgdaFunction{OnRoad}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{OnRoad}\AgdaSpace{}%
\AgdaBound{s}%
\>[295I]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∣}}\AgdaSpace{}%
\AgdaField{position}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∣}}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaFunction{3ℚ}\<%
\end{code}

==> agda/validObservation.tex <==
\begin{code}%
\>[0]\AgdaFunction{ValidObservation}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{Observation}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{ValidObservation}\AgdaSpace{}%
\AgdaBound{o}%
\>[295I]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∣}}\AgdaSpace{}%
\AgdaField{sensorError}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∣}}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaFunction{0.25ℚ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∣}}\AgdaSpace{}%
\AgdaField{windShift}\AgdaSpace{}%
\AgdaBound{o}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∣}}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaFunction{1ℚ}\<%
\end{code}

==> figures/generic-semantics.tex <==
\begin{gather*}
\ssemprog{[]} \triangleq \semTypeCtx
%
\semSpace
%
\ssemprog{\cons{\hDefType{f}{\gtype}}{\gprog}} \triangleq \ssemprog[\semNetworkCtx, \semDatasetCtx, \updatedCtx{\semKindCtx}{f}{\ssemtype{\gtype}}, \semTypeCtx]{p}
%
\\
%
\ssemprog{\cons{\hDef{f}{\gtype}{\gexpr}}{\gprog}} \triangleq \ssemprog[\semNetworkCtx, \semDatasetCtx,\semKindCtx,\updatedCtx{\semTypeCtx}{f}{\ssem{\gexpr}}]{p}
%
\semSpace
%
\ssemprog{\cons{\hNetworkDecl{f}{\gtype}}{\gprog}} \triangleq \ssemprog[\semNetworkCtx, \semDatasetCtx, \semKindCtx,\updatedCtx{\semTypeCtx}{f}{\semNetworkCtx[f]}]{p}
%
\\
%
\ssemprog{\cons{\hDatasetDecl{f}{\gtype}}{\gprog}} \triangleq \ssemprog[\semNetworkCtx, \semDatasetCtx, \semKindCtx,\updatedCtx{\semTypeCtx}{f}{\semDatasetCtx[f]}]{p}
%
\semSpace
%
\ssemprog{\cons{\hPropertyDecl{f}{\gexpr}}{\gprog}} \triangleq \ssemprog[\semNetworkCtx, \semDatasetCtx,\semKindCtx,\updatedCtx{\semTypeCtx}{f}{\ssem{\gexpr}}]{p}
\end{gather*}
\hrule
\begin{gather*}
\ssemtype{\hFunType{\gtype_1}{\gtype_2}} \triangleq \funInterpApp{\ssemtype{\gtype_1}}{ \monApp{(\ssemtype{\gtype_2})}}
%
\semSpace
%
\ssemtype{\hPi{\gvar}{\hNatKind}{\gtype}} \triangleq \piInterp (\lam{n}{\monApp{(\ssemtype[\updatedCtx{\kindCtx}{x}{n}]{\gtype})})}
%
\semSpace
%
\ssemtype{\gvar} \triangleq \semKindCtx[\gvar]
%
\\
%
\ssemtype{n} \triangleq n
%
\semSpace
%
\ssemtype{\hBoolType} \triangleq \boolInterp
%
\semSpace
%
\ssemtype{\hRealType} \triangleq \realInterp
%
\semSpace
%
\ssemtype{\hVecType{\gtype_1}{\gtype_2}} \triangleq
\funInterpApp{\hApp{\indexInterp}{{\ssem{\gtype_2}}}}{\monApp{(\ssemtype{\gtype_1})}}
%
\\
%
\ssemtype{\hIndexType{\gtype}} \triangleq \hApp{\indexInterp}{\ssemtype{\gtype}}
\end{gather*}
\hrule
\begin{gather*}
\ssem{\hApp{\gexpr_1}{\gexpr_2}} \triangleq \ssem{\gexpr_1} \ssem{\gexpr_2}
%
\semSpace
%
\ssem{\hLam{\gvar}{\gtype}{\gexpr}} \triangleq \lambda v . \ssem[\semKindCtx, \updatedCtx{\semTypeCtx}{\gvar}{v}]{\gexpr}
%
%\semSpace
%
%\ssem{\hLet{\gvar}{\gtype}{\gexpr_1}{\gexpr_2}} \triangleq \ssem[\updatedCtx{\semTypeCtx}{\gvar}{\ssem{e1}}]{e2}
%
\semSpace
%
\ssem{\gvar} \triangleq \semTypeCtx[\gvar]
%
\\
%
\ssem{r} \triangleq r
%
\semSpace
%
\ssem{\hTrue} \triangleq \trueInterp
%
\semSpace
%
\ssem{\hFalse} \triangleq \falseInterp
%
\semSpace
%
\ssem{\hAdd{\gexpr_1}{\gexpr_2}} \triangleq \addInterp \ssem{\gexpr_1} \ssem{\gexpr_2}
%
\\
%
\ssem{\hMul{\gexpr_1}{\gexpr_2}} \triangleq \mulInterp \ssem{\gexpr_1} \ssem{\gexpr_2}
%
\semSpace
%
\ssem{\hAt{\gexpr_1}{\gexpr_2}} \triangleq (\ssem{\gexpr_1})_{\ssem{\gexpr_2}}
%
\semSpace
%
\ssem{\hNot{\gexpr}} \triangleq \notInterp \ssem{\gexpr}
%
\\
%
\ssem{\hAnd{\gexpr_1}{\gexpr_2}} \triangleq \andInterp \ssem{\gexpr_1} \ssem{\gexpr_2}
%
\semSpace
%
\ssem{\hOr{\gexpr_1}{\gexpr_2}} \triangleq \orInterp \ssem{\gexpr_1} \ssem{\gexpr_2}
%
\\
%
\ssem{\hEq{\gexpr_1}{\gexpr_2}} \triangleq \eqInterp \ssem{\gexpr_1} \ssem{\gexpr_2}
%
\semSpace
%
\ssem{\hNeq{\gexpr_1}{\gexpr_2}} \triangleq \neqInterp \ssem{\gexpr_1} \ssem{\gexpr_2}
%
\\
%
\ssem{\hLeq{\gexpr_1}{\gexpr_2}} \triangleq \leqInterp \ssem{\gexpr_1} \ssem{\gexpr_2}
%
\semSpace
%
\ssem{\hLe{\gexpr_1}{\gexpr_2}} \triangleq \leInterp \ssem{\gexpr_1} \ssem{\gexpr_2}
%
\\
%
\ssem{\hIf{\gexpr_1}{\gexpr_2}{\gexpr_3}} \triangleq ???
\end{gather*}

==> figures/loss-semantics.tex <==

\begin{displaymath}
  \begin{array}{lcl}
\boolInterp &\triangleq & \real_{\infty}
%
\\
%
\trueInterp &\triangleq & \infty
%
\\
%
\falseInterp &\triangleq & -\infty
%
\\
%
\notInterp &\triangleq & \lam{x}{- x} 
%
\\
%
\andInterp &\triangleq &  \max
%
\\
%
\orInterp &\triangleq & \min
%
\\
%
\leqInterp &\triangleq & \lam{x y}{x - y} 
%
\\
%
\eqInterp & \triangleq & \lam{x y}{x \leqInterp y \wedge y \leqInterp x} 
%
\\
%
\ifInterp & \triangleq & \lam{c x y}{\begin{cases} x & c \geq 0 \\ y & otherwise \end{cases}}
%
\\
%
\forallInterp & \triangleq & \lam{f}{\max_{v \in \lsemtype{\gtype}} \lsem[\updatedCtx{\semTypeCtx}{\gvar}{v}]{f(v)}}
\\
%
\existsInterp & \triangleq & \min_{v \in \lsemtype{\gtype}} \lsem[\updatedCtx{\semTypeCtx}{\gvar}{v}]{\gexpr}
  \end{array}
%
\ssemprog{\cons{\hPropertyDecl{f}{\gexpr}}{\gprog}} \triangleq \ssemprog[\updatedCtx{\semTypeCtx}{f}{\ssem{\gexpr}}]{p}
\end{displaymath}

==> figures/marabou-syntax.tex <==
\centering
\begin{subfigure}{0.47\textwidth}
    \begin{grammar}
<prog>  ::= \lProg{[\queryClass]}

<query> ::= \lQuery{[\conjClass]}

<conj> ::= $\arithClass \compareClass \realClass$
 
<comp> ::= \eqSymbol{} | \neqSymbol{} | \leqSymbol{} | \leSymbol{}

<arith> ::= \lAdd{\arithClass}{\arithClass}
| \lMul{\realClass}{\varClass}

<var> ::= \lInputVar{\natClass} | \lOutputVar{\natClass}

<real> ::= $\lReal \in \real$

<nat> ::= $i \in \nat$
\end{grammar}
\end{subfigure}


==> figures/robustness-spec.tex <==
\hDefType{\hVar{Image}}{\hVecType{\hRealType{}}{10000}}
\\
\\
\hDefType{\hVar{Label}}{\hIndexType{10}}
\\
\\
\hDef{\hVar{epsilon}}{\hRealType}{0.1}
\\
\\
\hNetworkDecl{\hVar{f}}{\hFunType{\hVar{Image}}{\hVecType{\hRealType}{10}}}
\\
\\
\hDef{\hVar{validImage}}{\hFunType{\hVar{Image}}{\hBoolType}}{\hLam{x}{\hVar{Image}}{}}
\\
\\
\hDef{\hVar{validPerturbation}}{\hFunType{\hVar{Image}}{\hBoolType}}{\hLam{x}{\hVar{Image}}{}}
\\
\\
\hDef{\hVar{robustAround}}
{
\hFunType{\hVar{Image}}{\hFunType{\hVar{Label}}{\hBoolType}}
}
{
	\\ \hLam{x}{\hVar{Image}}{\hLam{i}{\hVar{Label}}		
	{
	\\ \hForall{\hVar{perturbation}}		{\hVecType{\hRealType}{10000}}
		{
			\\ \hImplies{\hAnd{\hApp{\hVar{validImage}}{(\hAdd{x}{\hVar{perturbation}})}}{\hApp{\hVar{validPerturbation}}{\hVar{perturbation}}}
		}{}
		}
	}
}}
\\
\\
\hDatasetDecl{\hVar{trainImages}}{\hVecType{\hVar{Image}}{100}}
\\
\\
\hDatasetDecl{\hVar{trainLabels}}{\hVecType{\hVar{Label}}{100}}
\\
\\
\hPropertyDecl{\hVar{robust}}{\hApp{\hApp{\hVar{robustAround}}{(\hAt{\hVar{trainImages}}{0})}}{(\hAt{\hVar{trainLabels}}{0})}}

==> figures/specification-diagram2.tex <==
	\newcommand{\drawTool}[4]
	{
		% NodeName
		% Purpose
		% Example text
		% Location
		\node(#1Top) [draw, rectangle, minimum width=4cm, align=center, fill=blue!30] at (#4) {#2};
		\node(#1Bottom) [draw, rectangle, minimum width=4cm, align=center, anchor=north] at (#1Top.south) {#3};
	}
	
    \begin{tikzpicture}
    	[ node distance=0.8cm and 1cm
    	]
	    \tikzstyle{middlebox}=[minimum width=1.5cm, minimum height=0.6cm] 
	    \tikzstyle{bigbox}=[minimum width=4cm, minimum height=6cm]
	    \tikzstyle{line}=[draw]
		\def\middlegap{0.5cm}
		\def\arrowshift{0.1cm}
    
        % Overall structure
        \node (agent) [bigbox] at (-3, 0) {};
        \node (gap) [bigbox, left=1cm of agent] {};
        \node (environment) [bigbox, left=1cm of gap] {};
        \node[above=0cm of agent] {\textbf{Neural world}};
        \node[above=0cm of gap] {Embedding gap};
        \node[above=0cm of environment] {\textbf{Symbolic world}};
        
		% Embedding gap
		\node[draw, rectangle, red, line width=0.5mm, minimum width=4.8cm, minimum height=6cm] (hidden) at (gap) {};
		\node (vehicle) at (gap) {\includegraphics[width=2cm]{figures/aisec-logo.png}};
		\node at (vehicle.south) {Our Vehicle tool};
        \node (spec) [draw, thick, minimum width=3cm, minimum height=0.6cm, below=0.35cm of gap.north] {Problem-space property, $\solutionProperty$};
		\node (verified) [draw, thick, minimum width=3.5cm, minimum height=0.6cm, above=0.35cm of gap.south] {Verified Model};
        
		
        % Four smaller boxes inside AI Neural Agent, aligned in a square
        \node (dataset) [middlebox, below=3*\middlegap of agent.north] {Dataset};
        \node (training) [middlebox, below=\middlegap of dataset] {Training};
        \node (verification) [middlebox, below=\middlegap of training] {Verification};
        \node (counterexamples) [middlebox, below=\middlegap of verification] {Counterexamples};
        
        \coordinate [xshift=0.3cm] (spec-coord) at (spec.east);
        \coordinate [xshift=0.3cm] (verified-coord) at (verified.east);
        
        % Arrows for cycle
        \draw[line,->] (dataset.south) -- (training.north);
        \draw[line,->] (training.south) -- (verification.north);
        \draw[line,->] (verification.south) -- (counterexamples.north);
        \draw[line,->] (counterexamples.east) -- ([xshift=0.3cm]counterexamples.east) |- (dataset.east);
        
        \draw[line] (spec.east) -- (spec-coord);
        \draw[line, ->] (spec-coord) |- (training);
        \draw[line, ->] (spec-coord) |- (verification.west);
        \draw[line] (verification.east) -| (verified-coord);
        \draw[line,->] (verified-coord) -- (verified);

		

        
        % World Model box inside Environment
        \drawTool{itp}{Verification of $\systemProperty(\system(u \circ f \circ e))$}{Via ITPs such as \\ Rocq, Agda, \\ Lean, KeYmaeraX etc.}{environment};
        
        \node (worldmodel) [draw, thick, minimum width=2cm, minimum height=0.6cm, below=0.35cm of environment.north] {System model, $\system$};
        
        \node (safety-proof) [draw, thick, minimum width=3.5cm, minimum height=0.6cm, above=0.5cm of environment.south] {Safety proof};        
        \coordinate [xshift=-0.3cm] (world-coord) at (worldmodel.west);
        \coordinate [xshift=0.3cm] (safety-coord) at ([yshift=\arrowshift]safety-proof.east);
        
		\draw[] ([yshift=\arrowshift]safety-proof.east) -- (safety-coord);
		%\draw[line,->] (safety-coord) |- (itps.east);
		%\draw[line,->] (world-coord) |- (itps.west);
        
        \draw[line,->] (worldmodel.south) -- (itpTop.north);
        \draw[dashed] ([xshift=-0.55cm,yshift=0.7cm]agent.north west) -- ([xshift=-0.55cm]agent.south west);
        \draw[line,->] (worldmodel.east) -- (spec.west);
        \draw[line,->] (verified.west) -- (safety-proof.east);
        
        %\draw[line,->, red, line width=0.5mm] (vehicle.west) -- (hidden.east);
    \end{tikzpicture}

==> figures/standard-semantics.tex <==
\begin{gather*}
\typeInterp \triangleq \text{Set}
%
\semSpace
%
\morphism \triangleq \rightarrow
%
\semSpace
%
\productInterp \triangleq \times
%
\semSpace
%
\initialInterp \triangleq ???
%
\semSpace
%
\funInterp \triangleq \rightarrow
%
\\
%
\piInterp \triangleq \lam{A}{\forall n . A n}
%
\semSpace
%
\mon \triangleq id
\\
%
\\
%
\\
%
\realInterp \triangleq \real
%
\semSpace
%
\realConstInterp \triangleq id
%
\semSpace
%
\addInterp \triangleq +
%
\semSpace
%
\mulInterp \triangleq \times
%
\\
%
\boolInterp \triangleq \bool
%
\semSpace
%
\trueInterp \triangleq \top
%
\semSpace
%
\falseInterp \triangleq \bot
%
\\
%
\notInterp \triangleq \neg
%
\semSpace
%
\andInterp \triangleq \wedge
%
\semSpace
%
\orInterp \triangleq \vee
%
\\
%
\eqInterp \triangleq \:\: = 
%
\semSpace
%
\neqInterp \triangleq \:\: \neq
%
\semSpace
%
\leqInterp \triangleq \:\: \leq
%
\semSpace
%
\leInterp \triangleq \:\: <
%
\\
%
\ifInterp \triangleq \lam{c, x, y}{\begin{cases}
x & \text{if }c \\
y & \text{otherwise}
\end{cases}}
%
\semSpace
%
\forallInterp \triangleq ???
%
\semSpace
%
\existsInterp \triangleq ???
%
\\
%
\indexInterp \triangleq \lam{n}{\{ 0, ..., n-1 \}}
%
\semSpace
%
\indexConstInterp \triangleq id
%
\semSpace
\end{gather*}

==> figures/vehicle-typing-rules.tex <==
\newcommand{\gap}{1em}
\begin{center}
\begin{gather*}
\infer
{
\hphantom{}
}
{
\progRel{[]}
}
%
\semSpace
%
\infer
{
\kindRel{\gtype}{\typeSymbol{}} \\ 
\progRel[\updatedCtx{\kindCtx}{f}{\gtype}, \typeCtx]{\gprog}
}
{
\progRel{\cons{(\hDefType{t}{\gtype})}{p}}
}
%
\\
%
\infer
{
\kindRel{\gtype}{\typeSymbol{}} \\ \typeRel{\gexpr}{\gtype} \\
\progRel[\kindCtx, \updatedCtx{\typeCtx}{f}{\gtype}]{\gprog}
}
{
\progRel{\cons{(\hDef{f}{\gtype}{\gexpr})}{p}}
}
%
\\
%
\infer
{
\exists m,n : \gtype = \hFunType{\hVecType{\hRealType}{m}}{\hVecType{\hRealType}{n}} \\
\kindRel{\gtype}{\typeSymbol{}} \\
\progRel[\kindCtx, \updatedCtx{\typeCtx}{f}{\gtype}]{\gprog}
}
{
\progRel{\cons{(\hNetworkDecl{f}{\gtype})}{p}}
}
%
\\
%
\infer
{
\exists n : \gtype = \hVecType{\hRealType}{n} \\
\kindRel{\gtype}{\typeSymbol{}} \\
\progRel[\kindCtx, \updatedCtx{\typeCtx}{f}{\gtype}]{\gprog}
}
{
\progRel{\cons{(\hDatasetDecl{f}{\gtype})}{p}}
}
%
\\
%
\infer
{
\typeRel{\gexpr}{\hBoolType} \\
\progRel[\kindCtx, \updatedCtx{\typeCtx}{f}{\hBoolType}]{\gprog}
}
{
\progRel{\cons{(\hPropertyDecl{f}{\gexpr})}{p}}
}
\end{gather*}
\vspace{\gap}
\hrule
\vspace{\gap}
\begin{gather*}
\infer{
\kindRel[\updatedCtx{\kindCtx}{\gvar}{\hNatKind}]{\gtype}{\hType}
}
{
\kindRel{\hPi{\gvar}{\hNatKind}{\gtype}}{\hType}
}
%
\semSpace
%
\infer
{
\kindCtx[\gvar] = \gkind
}
{
\kindRel{\gvar}{\gkind}
}
%
\semSpace
%
\infer
{
n \in \nat
}
{
\kindRel{n}{\hNatKind}
}
%
\semSpace
%
\infer
{
\hphantom{}
}
{
\kindRel{\hBoolType}{\hType}
}
%
\\
%
\infer
{
\kindRel{\gtype_1}{\hType} \\ 
\kindRel{\gtype_2}{\natSymbol{}}
}
{
\kindRel{\hVecType{\gtype_1}{\gtype_2}}{\hType}
}
%
\semSpace
%
\infer
{
\kindRel{\gtype}{\natSymbol{}}
}
{
\kindRel{\hIndexType{\gtype}}{\hType}
}
%
\semSpace
%
\infer
{
\hphantom{}
}
{
\kindRel{\hRealType}{\hType}
}
\end{gather*}
\vspace{\gap}
\hrule
\vspace{\gap}
\begin{gather*}
\infer
{
\typeRel[\updatedCtx{\kindCtx}{\gvar}{\gkind}, \typeCtx]{\gexpr}{\gtype}
}
{
\typeRel{\hAbs{\gvar}{\gkind}{\gexpr}}{\hPi{\gvar}{\gkind}{\gtype}}
}
%
\semSpace
%
\infer
{
\typeRel{\gexpr}{\hPi{\gvar}{\hNatKind}{\gtype_2}} \\ 
\kindRel{\gtype_2}{\hNatKind}
}
{
\typeRel{\hAbsApp{\gexpr}{\gtype_1}}{\gtype_2}
}
%
\\
%
\infer
{
\typeRel[\kindCtx, \updatedCtx{\typeCtx}{\gvar}{\gtype_1}]{\gexpr}{\gtype_2}
}
{
\typeRel{\hLam{\gvar}{\gtype_1}{\gexpr}}{\hFunType{\gtype_1}{\gtype_2}}
}
%
\semSpace
%
\infer
{
\typeRel{\gexpr_1}{\hFunType{\gtype_1}{\gtype_2}} \\ 
\typeRel{\gexpr_2}{\gtype_1}
}
{
\typeRel{\hApp{\gexpr_1}{\gexpr_2}}{\gtype_2}
}
%%
%\semSpace
%%
%\infer
%{
%\typeRel{e_1}{\tau_1} \\ \typeRel[\kindCtx, \updatedCtx{\typeCtx}{\gvar}{\gtype_1}]{e_2}{\tau_2}
%}
%{
%\typeRel{\hLet{\gvar}{\gtype_1}{\gexpr_1}{\gexpr_2}}{\gtype_2}
%}
%
\semSpace
%
\infer
{
\typeCtx[\gvar] = \gtype
}
{
\typeRel{\gvar}{\gtype}
}
%
\\
%
\infer
{
r \in \real
}
{
\typeRel{r}{\hRealType}
}
%
\semSpace
%
\infer
{
i \in \nat \\ i < n
}
{
\typeRel{i}{\hIndexType{n}}
}
%%
%\semSpace
%%
%\infer
%{
%\typeRel{\gexpr_1}{\hRealType} \\
%\typeRel{\gexpr_2}{\hRealType}
%}
%{
%\typeRel{\hAdd{\gexpr_1}{\gexpr_2}}{\hRealType}
%}
%%
%\semSpace
%%
%\infer
%{
%\typeRel{\gexpr_1}{\hRealType} \\
%\typeRel{\gexpr_2}{\hRealType}
%}
%{
%\typeRel{\hMul{\gexpr_1}{\gexpr_2}}{\hRealType}
%}
%%
%\\
%%
%\infer
%{
%}
%{
%\typeRel{\hTrue}{\hBoolType}
%}
%%
%\semSpace
%%
%\infer
%{
%}
%{
%\typeRel{\hFalse}{\hBoolType}
%}
%%
%\semSpace
%%
%\infer
%{
%\typeRel{\gexpr}{\hBoolType}
%}
%{
%\typeRel{\hNot{\gexpr}}{\hBoolType}
%}
%
%\semSpace
%
%\infer
%{
%\typeRel{\gexpr_1}{\hBoolType} \\
%\typeRel{\gexpr_2}{\hBoolType}
%}
%{
%\typeRel{\hAnd{\gexpr_1}{\gexpr_2}}{\hBoolType}
%}
%%
%\\
%%
%\infer
%{
%\typeRel{\gexpr_1}{\hBoolType} \\
%\typeRel{\gexpr_2}{\hBoolType}
%}
%{
%\typeRel{\hOr{\gexpr_1}{\gexpr_2}}{\hBoolType}
%}
%%
%\semSpace
%%
%\infer
%{
%\typeRel{\gexpr_1}{\hBoolType} \\
%\typeRel{\gexpr_2}{\hBoolType}
%}
%{
%\typeRel{\hImplies{\gexpr_1}{\gexpr_2}}{\hBoolType}
%}
%%
%\semSpace
%%
%\infer
%{
%\typeRel{\gexpr_1}{\hRealType} \\
%\typeRel{\gexpr_2}{\hRealType}
%}
%{
%\typeRel{\bop{\gexpr_1}{\bowtie}{\gexpr_2}}{\hBoolType}
%}
%\\
%%
%\infer
%{
%\typeRel{\gexpr_1}{\hBoolType} \\
%\typeRel{\gexpr_2}{\gtype} \\
%\typeRel{\gexpr_3}{\gtype}
%}
%{
%\typeRel{\hIf{\gexpr_1}{\gexpr_2}{\gexpr_3}}{\gtype}
%}
%\\
%\\
%\infer[(vec)]{\typeRel{\Seq{e_1}{e_n}}{\VecType{n}}}{\typeRel{e_1}{\RealType} & \ldots & \typeRel{e_n}{\RealType}}
%\semSpace
%\infer[(lookup)]{\typeRel{\:\AtSymbol{}}{\FunType{\VecType{n}}{\FunType{\FinType{n}}{\RealType}}}}{}
%\\
\\
%
\infer
{
\typeRel[\kindCtx,\updatedCtx{\typeCtx}{\gvar}{\gtype}]{\gexpr}{\hBoolType} \\ \gtype \neq \hPi{y}{\gtype_1}{\gtype_2}
}
{
\typeRel{\hForall{\gvar}{\gtype}{\gexpr}}{\hBoolType}
}
%
\semSpace
%
\infer
{
\typeRel[\kindCtx,\updatedCtx{\typeCtx}{\gvar}{\gtype}]{\gexpr}{\hBoolType} \\ \gtype \neq \hPi{y}{\gtype_1}{\gtype_2}
}
{
\typeRel{\hExists{\gvar}{\gtype}{\gexpr}}{\hBoolType}
}
%
\\
%
\infer
{
\typeRel{\gexpr_1}{\gtype}
\\
\ldots
\\
\typeRel{\gexpr_n}{\gtype}
}
{
\typeRel{\hSeq{\gexpr_1, \ldots, \gexpr_n}}{\hVecType{\gtype}{n}}
}
%
\semSpace
%
\infer
{
\typeRel{\gexpr_1}{\hVecType{\gtype}{n}} \\
\typeRel{\gexpr_2}{\hIndexType{n}}
}
{
\typeRel{\hAt{\gexpr_1}{\gexpr_2}}{\gtype}
}
%
\\
%
\infer
{
\typeRel[\kindCtx,\updatedCtx{\typeCtx}{\gvar}{\hIndexType{n}}]{\gexpr}{\gtype}
}
{
\typeRel{\hForeach{\gvar}{n}{\gexpr}}{\hVecType{\gtype}{n}}
}
%
\semSpace
%
\infer
{
\typeRel{\gexpr_1}{\hFunType{\hFunType{\gtype_1}{\gtype_2}}{\gtype_2}} \\
\typeRel{\gexpr_2}{\gtype_2} \\
\typeRel{\gexpr_3}{\hVecType{\gtype_1}{n}}
}
{
\typeRel{\hFold{\gexpr_1}{\gexpr_2}{\gexpr_3}}
}
\end{gather*}
\end{center}

==> figures/verifier-compilation-scaling.tex <==
\begin{tikzpicture}
\begin{axis}[
    xlabel={Number of inputs},
    ylabel={Mean compilation time (s)},
    xmin=0, xmax=10000,
    ymin=0, ymax=40,
    xtick={0,2000,4000,6000,8000,10000},
    ytick={0,10,20,30,40},
    legend pos=north east,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (1,0.1497)(100,0.3722)(400,1.3490)(900,4.3920)(1600,12.0910)(2500,35.6590)
    };
    \addlegendentry{Without optimisation}
    
\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (1,0.1562)(100,0.2491)(400,0.5109)(900,0.9860)(1600,1.6480)(2500,2.5680)(3600,3.8270)(4900,5.2190)(6400,6.6550)(8100,8.8270)(10000,11.4790)
    };
    \addlegendentry{With optimisation}
\end{axis}
\end{tikzpicture}

==> figures/verifier-syntax.tex <==

\centering
\begin{subfigure}[t]{0.32\textwidth}
\begin{grammar}
<prog> ::= [] | \cons{d}{\gprog}

<decl> $\ni d$ ::= \phantom{}
	\alt \hDefType{\identClass}{\gtype}
	\alt \hDef{\identClass}{\gtype}{\gexpr}
	\alt \hNetworkDecl{\identClass}{\gtype}
	\alt \hDatasetDecl{\identClass}{\gtype}
	\alt \hParameterDecl{\identClass}{\gtype}
	\alt \hPropertyDecl{\identClass}{\gtype}{\gexpr}

\end{grammar}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.65\textwidth}
\begin{grammar}
<kind> $\ni k$ ::= 
	\hType{}
	| \hNatKind{}
        | \hNumKind{}
        | \hBoolKind{}

<type> $\ni \gtype$ ::= 
	$\hPi{\gvar}{k}{\gtype}$
	| $\gvar$ 
	| $\hFunType{\gtype}{\gtype}$
	| $n \in \nat$
	| \hVecType{\gtype}{\gtype}
	| \hIndexType{\gtype}
	| \hBoolType
	| \hRealType

<expr> $\ni e$ ::=  
	$\hAbs{\gvar}{\gkind}{\gexpr}$
	| $\hAbsApp{\gexpr}{\gtype}$
	| $\hLam{\gvar}{\gtype}{\gexpr}$
	| $\hApp{\gexpr}{\gexpr}$
	% | $\hLet{\gvar}{\gtype}{e}{e}$
	| $\gvar$
	| $r \in \real$ 
	| \hAdd{\gexpr}{\gexpr}  
	| \hMul{\gexpr}{\gexpr}  
	| \hTrue{}
	| \hFalse{}
	| \hNot{\gexpr}
	| \hAnd{\gexpr}{\gexpr}
	| \hOr{\gexpr}{\gexpr}
	| \hEq{\gexpr}{\gexpr}
	| \hNeq{\gexpr}{\gexpr} 
	| \hLeq{\gexpr}{\gexpr}
	| \hLe{\gexpr}{\gexpr}
	| \hIf{\gexpr}{\gexpr}{\gexpr}
	| \hForall{\gvar}{\gtype}{\gexpr}
	| \hExists{\gvar}{\gtype}{\gexpr}
	| $i \in \nat$
	| \hSeq{\gexpr, $\ldots$, \gexpr}
	| \hAt{\gexpr}{\gexpr}
	| \hForeach{\gvar}{n}{\gexpr}
	| \hFold{\gexpr}{\gexpr}{\gexpr}
\end{grammar}
\end{subfigure}
